In-depth direct imaging and spectroscopic characterization of the young Solar System analog HD 95086

Context. HD 95086 is a young nearby Solar System analog hosting a giant exoplanet orbiting at 57 au from the star between an inner and outer debris belt. The existence of additional planets has been suggested as the mechanism that maintains the broad cavity between the two belts. Aims. We present a dedicated monitoring of HD 95086 with the VLT/SPHERE instrument to refine the orbital and atmospheric properties of HD 95086 b, and to search for additional planets in this system. Methods. SPHERE observations, spread over ten epochs from 2015 to 2019 and including five new datasets, were used. Combined with archival observations, from VLT/NaCo (2012-2013) and Gemini/GPI (2013-2016), the extended set of astrometric measurements allowed us to refine the orbital properties of HD 95086 b. We also investigated the spectral properties and the presence of a circumplanetary disk around HD 95086 b by using the special fitting tool exploring the diversity of several atmospheric models. In addition, we improved our detection limits in order to search for a putative planet c via the K-Stacker algorithm. Results. We extracted for the first time the JH low-resolution spectrum of HD 95086 b by stacking the six best epochs, and confirm its very red spectral energy distribution. Combined with additional datasets from GPI and NaCo, our analysis indicates that this very red color can be explained by the presence of a circumplanetary disk around planet b, with a range of high-temperature solutions (1400-1600 K) and significant extinction (Av > 10 mag), or by a super-solar metallicity atmosphere with lower temperatures (800-1300 K), and small to medium amount of extinction (Av < 10 mag). We do not find any robust candidates for planet c, but give updated constraints on its potential mass and location.

==> fig/inutile_corner_plot.tex <==
\section{Reduced images by the pipeline SpeCal}
\begin{comment}
%%%%%%%%%
%%%%%%%%%

\begin{figure*}[h!]
    \centering
    \includegraphics[width=1\linewidth]{fig/mosaic_IRDIS_TLOCI.pdf} 
    
    \vspace{0.1cm}
    
    \includegraphics[width=1\linewidth]{fig/mosaic_IFS_PCAPad.pdf}
    \caption{The signal-to-noise ratio (S/N) maps for all the SPHERE epochs: at the \textit{top}, IRDIS in the K1-band reduced by the pipeline SpeCal-TLOCI, and at the \textit{bottom}, IFS in the YJH-bands) reduced by the pipeline SpeCal-PCAPad (PCA ADI+SDI). The colorbar corresponds to the signal-to-noise ratio. The region below the inner working angle of the coronagraph is masked.}
    \label{fig:mosaic_epochs_specal}
\end{figure*}
\end{comment}

\begin{comment}
    \begin{figure*}[h!]
        \centering \vspace{0.5cm}
        \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IRDIS_cADI_Jan2018.pdf} 
        \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IRDIS_TLOCI_Jan2018.pdf} 
        \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IRDIS_PCA_Jan2018.pdf}
        \includegraphics[height=3.5cm,trim={0cm 0cm 0cm 0cm}, clip]{fig/ex_IRDIS_ANDROMEDA_Jan2018.pdf}
    
        
        %\smallskip
        
        \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IFS_cADI_Jan2018.pdf} 
        \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IFS_TLOCI_Jan2018.pdf} \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IFS_PCA_Jan2018.pdf} \includegraphics[height=3.5cm,trim={0cm 0cm 1.5cm 0cm}, clip]{fig/ex_IFS_PCAPad_Jan2018.pdf}
        \includegraphics[height=3.5cm,trim={0cm 0cm 0cm 0cm}, clip]{fig/ex_IFS_ANDROMEDA_Jan2018.pdf}
        \caption{The S/N maps for different algorithms for the epoch Jan2018: at the \textit{top} with IRDIS in K1-band and at the \textit{bottom} with IFS in YJH-bands or in the spectral channel 38 ($1.62~\mathrm{\mu m}$, i.e. H-band). The colorbar corresponds to the S/N.  The region below the inner working angle of the coronagraph is masked. At the top right-hand corner on IFS data, one can see one or two point-like features which actually corresponds to the remanence of the star during the flux calibration on the IFS detector. Note: $5$ modes have been used for PCA-ADI reductions.}
        \label{fig:reduction_comparaison_algo}
    \end{figure*}
\end{comment}

\begin{comment}
    \begin{figure*}[t]
        \centering
        \includegraphics[height=7cm]{fig/cc_IRDIS_Jan2018.pdf} \qquad \includegraphics[height=7cm]{fig/cc_IFS_Jan2018.pdf}
        \caption{Detection limits for IRDIS in the band K1 on the \textit{left} and IFS in the bands YJH on the \textit{right} regarding different post-processing algorithms (SpeCal-TLOCI in green dashed dotted line, SpeCal-cADI in orange dotted line, SpeCal-PCA ADI in pink solid line, SpeCal-PCA ASDI in red solid line, and ANDROMEDA in dashed blue line) for the epoch Jan2018. The gray area corresponds to the area hidden by the larger coronograph used for all the epochs (i.e. "N\_ALC\_Ks") which has an inner working angle of $0.107~"$ and $0.116~"$ for IFS and IRDIS, respectively. The blue vertical line correspond to the position of the planet HD~95086~b at the best epoch January 2018 (cyan, $0.625~\mathrm{"}$).  }
        \label{fig:contrast_curve_jan2018_comparaison_algo}
    \end{figure*}
\end{comment}

%\section*{Appendix B \label{app:B}}
%\section{Previous MCMC results for %NaCo and SPHERE data}
%\begin{figure*}[p]
%    \centering
%    \includegraphics[width=\linewidth]{fig/fig6.pdf}
%    \caption{Results from \citet{Chauvin2018} for the MCMC orbital fit of HD 95086 b based on the NaCo (2012-2013, band L', \citep{Rameau2013b}) and SPHERE (2015-2017, band K1, \citep{Chauvin2018}) astrometric data. The orbital fitting parameters are $t_p$, $w$ (\degr), $\Omega$ (\degr), $i$ (\degr), e. The red line in the histograms and the black star in the correlation plots represent the position of the best LSLM $\chi_r^2$ model. }
%    \label{fig:triangle_orbital_fit_previous}
%\end{figure*}
\begin{comment}
\section{Spectral correlation matrix}\label{app:SpectralCovariance}

Fig.~\ref{fig:covar_matrix} shows the spectral correlation matrix ($\phi$) empirically estimated from our IFS datasets as in \citet{Greco2016} and \citet{Derosa2016}. The spectral covariance matrix $C$  used for spectral fits is obtained as $C_{ij} = \phi_{ij} \sigma_i \sigma_j$, where $\sigma_i$ and $\sigma_j$ correspond to the reported uncertainties in flux measurements for points $i$ and $j$.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/spec_covar.pdf}
    \caption{Spectral correlation matrix computed from our SPHERE/IFS (first 15 points) and GPI/IFS (points \# 15 to 43) data. For IRDIS and NACO, $C_{ij} = \delta_{ij}$ where $\delta_{ij}$ is the Kroenecker symbol.}
    \label{fig:covar_matrix}
\end{figure*}
\end{comment}
%%%%%%%%
%%%%%%%%

\section{Corner plots of the posteriors of the atmospheric models}\label{app:cornerplots_special}

Figures \ref{fig:corner_plots_BT-Settl} to \ref{fig:corner_plot_M11cA_BB} show the corner plots of posteriors retrieved by \texttt{special} for some of the best models at reproducing the observed spectrum. In each case, the mass is not a free parameter of the fit, but is calculated from the $\log(g)$ and $R_\text{p}$ posterior distributions.

\newpage
test
\vfill

\newpage
test
\vfill

  
\begin{figure*}[h!]
    \centering
    
    \vspace{4cm}
     \includegraphics[width=\textwidth]{fig/BT-Settl_single_BB_corner_plot.pdf}
    \caption{Corner plots retrieved by \texttt{special} for the single blackbody model at the \textit{top-right}, BT-SETTL  with free extinction $A_v$ model at the \textit{bottom-left}.  
    (with free $A_V$), d) DRIFT-PHOENIX and e) \citetalias{Madhusudhan2011} cloud-A model with an extra blackbody component.}
    \label{fig:corner_plots_BT-Settl_BB}
\end{figure*}

\newpage

\begin{tikzpicture}[remember picture,overlay]

    \node[yshift=8.cm,xshift=4cm] at (current page.center){%
    
     \includegraphics[width=0.48\textwidth]{fig/BB_corner_plot.pdf}};
  \end{tikzpicture}
  
\begin{figure*}[h!]
    \centering
     \includegraphics[width=\textwidth]{fig/DP_corner_plot_withM.pdf}
    \caption{Corner plot retrieved by \texttt{special} for the DRIFT-PHOENIX model with free extinction $A_v$. }
    \label{fig:corner_plots_DP}
\end{figure*}

\begin{figure*}[h!]
    \centering
     \includegraphics[width=\textwidth]{fig/M11A_corner_plot_withM.pdf}
    \caption{Corner plot retrieved by \texttt{special} for the \citetalias{Madhusudhan2011} cloud-A model with free extinction $A_v$. }
    \label{fig:corner_plot_M11cA}
\end{figure*}


\begin{figure*}[h!]
    \centering
     \includegraphics[width=\textwidth]{fig/M11A_BB_corner_plot_withM.pdf}
    \caption{Corner plot retrieved by \texttt{special} for the \citetalias{Madhusudhan2011} cloud-A model with free extinction $A_v$ and with an extra blackbody component. }
    \label{fig:corner_plot_M11cA_BB}
\end{figure*}


\begin{comment}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{fig/Corner_plots_v3.pdf}
    \caption{Corner plots retrieved by \texttt{specfit} for some of the best models at reproducing the observed spectrum: a) single blackbody, b) \citetalias{Madhusudhan2011} cloud-A model, c) BT-SETTL (with free $A_V$), d) DRIFT-PHOENIX and e) \citetalias{Madhusudhan2011} cloud-A model with an extra blackbody component. The mass is not a free parameter of the fit, but is calculated from the $\log(g)$ and $R_\text{p}$ posterior distributions.}
    \label{fig:corner_plots}
\end{figure*}
\end{comment}
